Grammar-compressed Self-index with Lyndon Words

We introduce a new class of straight-line programs (SLPs), named the Lyndon SLP, inspired by the Lyndon trees (Barcelo, 1990). Based on this SLP, we propose a self-index data structure of $O(g)$ words of space that can be built from a string $T$ in $O(n \lg n)$ expected time, retrieving the starting positions of all occurrences of a pattern $P$ of length $m$ in $O(m + \lg m \lg n + occ \lg g)$ time, where $n$ is the length of $T$, $g$ is the size of the Lyndon SLP for $T$, and $occ$ is the number of occurrences of $P$ in $T$.

==> mergedtable.tex <==

\begin{tabular}{l|c*{4}{r}}
    \hline \hline
    \multicolumn{1}{c|}{collection} &
    \multicolumn{1}{c}{} &
    \multicolumn{1}{c}{Re-Pair} &
    \multicolumn{1}{c}{ESP} &
    \multicolumn{1}{c}{Recompression} &
    \multicolumn{1}{c}{LyndonSLP} \\
    \hline
    \texttt{cere}
    & SLP & 6,433,178 & 10,835,450 & 8,537,742 & 13,026,556 \\
    & AG  & 5,777,882 &            & 5,309,784 & 7,469,983 \\
    \hline
    \texttt{einstein.de.txt}
    & SLP & 125,226 & 269,256 & 202,632 & 205,230 \\
    & AG  & 112,563 &         & 127,673 & 124,044 \\
    \hline
    \texttt{einstein.en.txt}
    & SLP & 326,166 & 694,350 & 536,330 & 699,110 \\
    & AG  & 263,695 &         & 323,473 & 394,803 \\
    \hline
    \texttt{Escherichia\_coli}
    & SLP & 7,227,136 & 10,377,252 & 8,945,368 & 11,320,990 \\
    & AG  & 5,625,656 &            & 5,305,946 & 6,460,386 \\
    \hline
    \texttt{influenza}
    & SLP & 3,060,844 & 5,511,898 & 4,195,248 & 5,349,394 \\
    & AG  & 2,174,010 &           & 2,524,915 & 3,055,435 \\
    \hline
    \texttt{kernel}
    & SLP & 2,254,680 & 4,362,082 & 3,587,222 & 4,201,734 \\
    & AG  & 2,185,255 &           & 2,135,619 & 2,400,327 \\
    \hline
    \texttt{para}
    & SLP & 8,483,044 & 13,873,376 & 11,297,212 & 15,519,192 \\
    & AG  & 7,335,396 &            & 7,009,052 & 9,022,051 \\
    \hline
    \texttt{world\_leaders}
    & SLP & 601,668 & 1,336,410 & 1,023,650 & 911,132 \\
    & AG  & 507,343 &           & 636,611 & 552,573 \\
    \hline
\end{tabular}


